Geospatial Disparities: A Case Study on Real Estate Prices in Paris

Driven by an increasing prevalence of trackers, ever more IoT sensors, and the declining cost of computing power, geospatial information has come to play a pivotal role in contemporary predictive models. While enhancing prognostic performance, geospatial data also has the potential to perpetuate many historical socio-economic patterns, raising concerns about a resurgence of biases and exclusionary practices, with their disproportionate impacts on society. Addressing this, our paper emphasizes the crucial need to identify and rectify such biases and calibration errors in predictive models, particularly as algorithms become more intricate and less interpretable. The increasing granularity of geospatial information further introduces ethical concerns, as choosing different geographical scales may exacerbate disparities akin to redlining and exclusionary zoning. To address these issues, we propose a toolkit for identifying and mitigating biases arising from geospatial data. Extending classical fairness definitions, we incorporate an ordinal regression case with spatial attributes, deviating from the binary classification focus. This extension allows us to gauge disparities stemming from data aggregation levels and advocates for a less interfering correction approach. Illustrating our methodology using a Parisian real estate dataset, we showcase practical applications and scrutinize the implications of choosing geographical aggregation levels for fairness and calibration measures.

==> tikz/explainer_attributes.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Image [id:dp2580480893894639] 
\draw (89.67,134.5) node  {\includegraphics[width=54.5pt,height=64.75pt]{figs/explainers/img_celeba.png}};
%Shape: Square [id:dp024893756309259496] 
\draw  [fill={rgb, 255:red, 0; green, 80; blue, 173 }  ,fill opacity=1 ] (154.33,76.32) -- (185.19,76.32) -- (185.19,107.18) -- (154.33,107.18) -- cycle ;
%Shape: Rectangle [id:dp929520613452512] 
\draw  [fill={rgb, 255:red, 40; green, 76; blue, 0 }  ,fill opacity=1 ] (160.37,70.15) -- (191.23,70.15) -- (191.23,101.01) -- (160.37,101.01) -- cycle ;
%Shape: Square [id:dp7692738462862141] 
\draw  [fill={rgb, 255:red, 235; green, 25; blue, 25 }  ,fill opacity=1 ] (166.47,63.94) -- (197.33,63.94) -- (197.33,94.81) -- (166.47,94.81) -- cycle ;
%Straight Lines [id:da550622191490143] 
\draw    (210.67,177) -- (290.08,176.92) -- (290.08,131.25) ;
\draw [shift={(290.08,129.25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3816021885213434] 
\draw    (209.5,142.25) -- (270.75,142.25) -- (270.61,130.58) ;
\draw [shift={(270.58,128.58)}, rotate = 89.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3053781296586149] 
\draw    (199.83,79.67) -- (249.75,79.58) -- (249.59,107.75) ;
\draw [shift={(249.58,109.75)}, rotate = 270.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (150,167.4) node [anchor=north west][inner sep=0.75pt]    {$\{\text{Young} \}$};
% Text Node
\draw (147,132.73) node [anchor=north west][inner sep=0.75pt]    {$\{\text{Female} \}$};
% Text Node
\draw (151.33,111.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {Image Tensor};
% Text Node
\draw (234.33,109.9) node [anchor=north west][inner sep=0.75pt]    {$(\boldsymbol{X} ,\ S,\ Y)$};


\end{tikzpicture}

\vspace{-1cm}

==> tikz/interpretation.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da34493428190958975] 
\draw    (101.01,59.1) -- (101.01,179.5) ;
%Straight Lines [id:da5610744170520812] 
\draw    (101.01,179.5) -- (339.93,179.77) ;
%Curve Lines [id:da18793005073064073] 
\draw [color={rgb, 255:red, 224; green, 65; blue, 65 }  ,draw opacity=1 ][line width=1.5]   (101.01,179.5) .. controls (306.6,186.43) and (191.6,77.1) .. (319.54,71.09) ;
%Shape: Circle [id:dp34827496852575335] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 239; green, 10; blue, 10 }  ,fill opacity=1 ][line width=0.75]  (241.77,120.43) .. controls (241.77,119.14) and (242.81,118.1) .. (244.1,118.1) .. controls (245.39,118.1) and (246.43,119.14) .. (246.43,120.43) .. controls (246.43,121.72) and (245.39,122.77) .. (244.1,122.77) .. controls (242.81,122.77) and (241.77,121.72) .. (241.77,120.43) -- cycle ;
%Curve Lines [id:da299904411828978] 
\draw [color={rgb, 255:red, 2; green, 92; blue, 198 }  ,draw opacity=1 ] [line width=1.5]  (101.01,179.5) .. controls (239.6,144.43) and (137.93,72.43) .. (319.54,71.09) ;
%Shape: Circle [id:dp8287462651390198] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 23; green, 101; blue, 193 }  ,fill opacity=1 ][line width=0.75]  (186.77,120.43) .. controls (186.77,119.14) and (187.81,118.1) .. (189.1,118.1) .. controls (190.39,118.1) and (191.43,119.14) .. (191.43,120.43) .. controls (191.43,121.72) and (190.39,122.77) .. (189.1,122.77) .. controls (187.81,122.77) and (186.77,121.72) .. (186.77,120.43) -- cycle ;
%Shape: Boxed Line [id:dp23220239283834365] 
\draw    (244.39,122.77) -- (244.5,184.13) ;
%Straight Lines [id:da6397219432613375] 
\draw    (96.35,119.98) -- (186.77,120.43) ;
%Shape: Boxed Line [id:dp08046938788866398] 
\draw    (188.89,122.77) -- (189,204.2) ;
%Shape: Triangle [id:dp9898969051467064] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (101.01,59.1) -- (102.71,64.9) -- (99.31,64.9) -- cycle ;
%Shape: Triangle [id:dp49548946910857006] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (342.83,179.77) -- (337.03,181.47) -- (337.03,178.07) -- cycle ;
%Straight Lines [id:da1657941959836724] 
\draw[dashed] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (191.43,120.43) -- (241.77,120.43) ;
%Shape: Boxed Line [id:dp8044163695236335] 
\draw    (217.14,175.94) -- (217.25,228.38) ;
%Straight Lines [id:da3761853074214718] 
\draw[dashed] [color={rgb, 255:red, 81; green, 137; blue, 11 }  ,draw opacity=1 ]   (189.35,175.78) -- (217.14,175.94) ;

% Text Node
\draw (88.52,38.3) node [anchor=north west][inner sep=0.75pt]    {$F( x)$};
% Text Node
\draw (345,168.11) node [anchor=north west][inner sep=0.75pt]    {$f^{*}( x)$};
% Text Node
\draw (226.72,187.38) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$Q_{f^{*} |s=2}( F_{f^{*} |s=1}( f( x_{0} ,s=1)))$};
% Text Node
\draw (155.1,203.93) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$f(x_{0},s=1)$};
% Text Node
\draw (-15.97,115.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$F_{f^{*} |s=1}( f( x_{0} ,s=1))$};
% Text Node
\draw (192.05,231.53) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$f( x_{0} ,s=2)$};


\end{tikzpicture}


==> tikz/tikz_explainer.tex <==
\tikzset{every picture/.style={line width=0.5pt}} %set default line width to 0.75pt     

\tikzset{global scale/.style={
    scale=#1,
    every node/.style={scale=#1}
  }
}
% Gradient Info
  
\tikzset {_rttks5pci/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_zsnft31t3}{150bp}{rgb(0bp)=(0.38,0.38,0.39);
rgb(37.5bp)=(0.38,0.38,0.39);
rgb(54.01785714285714bp)=(0.87,0.87,0.87);
rgb(100bp)=(0.87,0.87,0.87)}
%\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\tikzset{every picture/.style={line width=0.5pt}} %set default line width to 0.75pt     

\tikzset{global scale/.style={
    scale=#1,
    every node/.style={scale=#1}
  }
}


%\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
\begin{tikzpicture}[x=0.65pt,y=0.65pt,yscale=-1,xscale=1]


%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp7528645092540092] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 89; green, 89; blue, 89 }  ,fill opacity=1 ] (70,70) -- (120,70) -- (120,180) -- (70,180) -- cycle ;
%Shape: Rectangle [id:dp9139334557404273] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 212; green, 212; blue, 212 }  ,fill opacity=1 ] (179,70) -- (204,70) -- (204,180) -- (179,180) -- cycle ;
%Shape: Triangle [id:dp8476139480228015] 
\draw  [draw opacity=0][shading=_zsnft31t3,_rttks5pci] (178.67,124.9) -- (120.33,143.07) -- (120.33,106.73) -- cycle ;
%Rounded Rect [id:dp44380759408064097] 
\draw   (221.4,143.12) .. controls (221.4,141.95) and (222.35,141) .. (223.52,141) -- (229.88,141) .. controls (231.05,141) and (232,141.95) .. (232,143.12) -- (232,156.88) .. controls (232,158.05) and (231.05,159) .. (229.88,159) -- (223.52,159) .. controls (222.35,159) and (221.4,158.05) .. (221.4,156.88) -- cycle ;
%Rounded Rect [id:dp5027159100469891] 
\draw   (221,94.12) .. controls (221,92.95) and (221.95,92) .. (223.12,92) -- (229.48,92) .. controls (230.65,92) and (231.6,92.95) .. (231.6,94.12) -- (231.6,107.88) .. controls (231.6,109.05) and (230.65,110) .. (229.48,110) -- (223.12,110) .. controls (221.95,110) and (221,109.05) .. (221,107.88) -- cycle ;
%Shape: Triangle [id:dp44172082517133315] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (191.33,64.3) -- (187.62,60.3) -- (195.08,60.3) -- cycle ;
%Shape: Triangle [id:dp35804770739538916] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (95.33,64.3) -- (91.62,60.3) -- (99.08,60.3) -- cycle ;
%Flowchart: Direct Access Storage [id:dp4632379178200281] 
\draw   (285.73,139) -- (256.48,139) .. controls (252.13,139) and (248.6,131.48) .. (248.6,122.2) .. controls (248.6,112.92) and (252.13,105.4) .. (256.48,105.4) -- (285.73,105.4)(293.6,122.2) .. controls (293.6,131.48) and (290.07,139) .. (285.73,139) .. controls (281.38,139) and (277.85,131.48) .. (277.85,122.2) .. controls (277.85,112.92) and (281.38,105.4) .. (285.73,105.4) .. controls (290.07,105.4) and (293.6,112.92) .. (293.6,122.2) ;
%Rounded Rect [id:dp28505864389303315] 
\draw   (310.6,143.32) .. controls (310.6,142.15) and (311.55,141.2) .. (312.72,141.2) -- (319.08,141.2) .. controls (320.25,141.2) and (321.2,142.15) .. (321.2,143.32) -- (321.2,157.08) .. controls (321.2,158.25) and (320.25,159.2) .. (319.08,159.2) -- (312.72,159.2) .. controls (311.55,159.2) and (310.6,158.25) .. (310.6,157.08) -- cycle ;
%Rounded Rect [id:dp629296498696893] 
\draw   (310.2,94.32) .. controls (310.2,93.15) and (311.15,92.2) .. (312.32,92.2) -- (318.68,92.2) .. controls (319.85,92.2) and (320.8,93.15) .. (320.8,94.32) -- (320.8,108.08) .. controls (320.8,109.25) and (319.85,110.2) .. (318.68,110.2) -- (312.32,110.2) .. controls (311.15,110.2) and (310.2,109.25) .. (310.2,108.08) -- cycle ;
%Shape: Triangle [id:dp004078876748576432] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (275.83,64.3) -- (272.12,60.3) -- (279.58,60.3) -- cycle ;
%Straight Lines [id:da0825169482613719] 
\draw    (204.3,101) -- (215,101) -- (217.5,101.14) ;
\draw [shift={(219.5,101.25)}, rotate = 183.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-2.3) .. controls (4.86,-0.97) and (2.31,-0.21) .. (0,0) .. controls (2.31,0.21) and (4.86,0.98) .. (7.65,2.3)   ;
%Straight Lines [id:da7856445660786735] 
\draw    (205.1,150.8) -- (215.8,150.8) -- (218.3,150.94) ;
\draw [shift={(220.3,151.05)}, rotate = 183.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-2.3) .. controls (4.86,-0.97) and (2.31,-0.21) .. (0,0) .. controls (2.31,0.21) and (4.86,0.98) .. (7.65,2.3)   ;
%Image [id:dp9391915499376811] 
\draw (227.38,232.38) node  {\includegraphics[width=66.56pt,height=35.81pt]{figs/explainers/uncorrected.png}};
%Image [id:dp4426968349169691] 
\draw (397.38,121) node  {\includegraphics[width=69.56pt,height=37.13pt]{figs/explainers/corrected.png}};

% Text Node
\draw (140,41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Classification Layer}
\end{center}

\end{minipage}};
% Text Node
\draw (45,41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60.88pt}\setlength\topsep{0pt}
\begin{center}
{\tiny (Pretrained) Embedding}
\end{center}

\end{minipage}};
% Text Node
\draw (212.4,176.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {${\textstyle \hat{f}(\boldsymbol{X} ,\ S)}$};
% Text Node
\draw (301.4,176.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {${\textstyle \hat{f}_{B}(\boldsymbol{X} ,\ S)}$};
% Text Node
\draw (230,41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60.28pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Calibration Layer}
\end{center}
\end{minipage}};

% Text Node
\draw (203.5,195.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.62pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Unfair Scores}
\end{center}

\end{minipage}};

\draw (373.5,75.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{28.79pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Fair Scores}
\end{center}

\end{minipage}};


\end{tikzpicture}

\vspace{-1cm}


==> tikz/tikz_explainer_2.tex <==


% Gradient Info
  
\tikzset {_fhv5kzqa5/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_ygqylz1us}{150bp}{rgb(0bp)=(0.38,0.38,0.39);
rgb(37.5bp)=(0.38,0.38,0.39);
rgb(54.01785714285714bp)=(0.87,0.87,0.87);
rgb(100bp)=(0.87,0.87,0.87)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% Gradient Info
  
\tikzset {_89j6skns2/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_oqycwsqdy}{150bp}{rgb(0bp)=(0.38,0.38,0.39);
rgb(37.5bp)=(0.38,0.38,0.39);
rgb(54.01785714285714bp)=(0.87,0.87,0.87);
rgb(100bp)=(0.87,0.87,0.87)}

% Gradient Info
  
\tikzset {_alay4xbbr/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_3ubsli8nm}{150bp}{rgb(0bp)=(0.38,0.38,0.39);
rgb(37.5bp)=(0.38,0.38,0.39);
rgb(54.01785714285714bp)=(0.87,0.87,0.87);
rgb(100bp)=(0.87,0.87,0.87)}

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp7528645092540092] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 89; green, 89; blue, 89 }  ,fill opacity=1 ] (70,70) -- (120,70) -- (120,180) -- (70,180) -- cycle ;
%Shape: Rectangle [id:dp9139334557404273] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 212; green, 212; blue, 212 }  ,fill opacity=1 ] (179,70) -- (204,70) -- (204,180) -- (179,180) -- cycle ;
%Shape: Triangle [id:dp8476139480228015] 
\draw  [draw opacity=0][shading=_ygqylz1us,_fhv5kzqa5] (178.67,123.41) -- (120.33,156.07) -- (120.33,90.75) -- cycle ;
%Rounded Rect [id:dp44380759408064097] 
\draw   (221.4,143.12) .. controls (221.4,141.95) and (222.35,141) .. (223.52,141) -- (229.88,141) .. controls (231.05,141) and (232,141.95) .. (232,143.12) -- (232,156.88) .. controls (232,158.05) and (231.05,159) .. (229.88,159) -- (223.52,159) .. controls (222.35,159) and (221.4,158.05) .. (221.4,156.88) -- cycle ;
%Rounded Rect [id:dp5027159100469891] 
\draw   (221,94.12) .. controls (221,92.95) and (221.95,92) .. (223.12,92) -- (229.48,92) .. controls (230.65,92) and (231.6,92.95) .. (231.6,94.12) -- (231.6,107.88) .. controls (231.6,109.05) and (230.65,110) .. (229.48,110) -- (223.12,110) .. controls (221.95,110) and (221,109.05) .. (221,107.88) -- cycle ;
%Shape: Triangle [id:dp44172082517133315] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (191.33,64.3) -- (187.62,60.3) -- (195.08,60.3) -- cycle ;

\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (356,99.5) -- (356,149.5) ;


%Shape: Triangle [id:dp35804770739538916] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (95.33,64.3) -- (91.62,60.3) -- (99.08,60.3) -- cycle ;
%Flowchart: Direct Access Storage [id:dp4632379178200281] 
\draw   (345.73,141) -- (316.48,141) .. controls (312.13,141) and (308.6,133.48) .. (308.6,124.2) .. controls (308.6,114.92) and (312.13,107.4) .. (316.48,107.4) -- (345.73,107.4)(353.6,124.2) .. controls (353.6,133.48) and (350.07,141) .. (345.73,141) .. controls (341.38,141) and (337.85,133.48) .. (337.85,124.2) .. controls (337.85,114.92) and (341.38,107.4) .. (345.73,107.4) .. controls (350.07,107.4) and (353.6,114.92) .. (353.6,124.2) ;
%Rounded Rect [id:dp28505864389303315] 
\draw   (373.1,143.12) .. controls (373.1,141.95) and (374.05,141) .. (375.22,141) -- (381.58,141) .. controls (382.75,141) and (383.7,141.95) .. (383.7,143.12) -- (383.7,156.88) .. controls (383.7,158.05) and (382.75,159) .. (381.58,159) -- (375.22,159) .. controls (374.05,159) and (373.1,158.05) .. (373.1,156.88) -- cycle ;
%Rounded Rect [id:dp629296498696893] 
\draw  (372.7,94.12) .. controls (372.7,92.95) and (373.65,92) .. (374.82,92) -- (381.18,92) .. controls (382.35,92) and (383.3,92.95) .. (383.3,94.12) -- (383.3,107.88) .. controls (383.3,109.05) and (382.35,110) .. (381.18,110) -- (374.82,110) .. controls (373.65,110) and (372.7,109.05) .. (372.7,107.88) -- cycle ;
%Shape: Triangle [id:dp004078876748576432] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (329.33,64.3) -- (325.62,60.3) -- (333.08,60.3) -- cycle ;
%Straight Lines [id:da0825169482613719] 
\draw    (204.3,101) -- (215,101) -- (217.5,101.14) ;
\draw [shift={(219.5,101.25)}, rotate = 183.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-2.3) .. controls (4.86,-0.97) and (2.31,-0.21) .. (0,0) .. controls (2.31,0.21) and (4.86,0.98) .. (7.65,2.3)   ;
%Straight Lines [id:da7856445660786735] 
\draw    (205.1,150.8) -- (215.8,150.8) -- (218.3,150.94) ;
\draw [shift={(220.3,151.05)}, rotate = 183.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-2.3) .. controls (4.86,-0.97) and (2.31,-0.21) .. (0,0) .. controls (2.31,0.21) and (4.86,0.98) .. (7.65,2.3)   ;
%Image [id:dp9391915499376811] 
\draw (265.63,123.25) node  {\includegraphics[width=45.19pt,height=24.75pt]{figs/explainers/uncorrected.png}};
%Image [id:dp4426968349169691] 
\draw (430.13,123.25) node  {\includegraphics[width=45.19pt,height=24.75pt]{figs/explainers/corrected.png}};
%Shape: Triangle [id:dp2898479153362763] 
\draw  [draw opacity=0][fill={rgb, 255:red, 86; green, 86; blue, 86 }  ,fill opacity=1 ] (305.75,123.91) -- (300.83,141.07) -- (300.83,106.75) -- cycle ;
%Straight Lines [id:da8693721364695837] 
\draw    (355.8,99.5) -- (366.5,99.5) -- (369,99.64) ;
\draw [shift={(371,99.75)}, rotate = 183.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-2.3) .. controls (4.86,-0.97) and (2.31,-0.21) .. (0,0) .. controls (2.31,0.21) and (4.86,0.98) .. (7.65,2.3)   ;
%Straight Lines [id:da928447014068521] 
\draw    (355.8,149) -- (367.5,149) -- (370,149.14) ;
\draw [shift={(372,149.25)}, rotate = 183.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-2.3) .. controls (4.86,-0.97) and (2.31,-0.21) .. (0,0) .. controls (2.31,0.21) and (4.86,0.98) .. (7.65,2.3)   ;

% Text Node
\draw (150,41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{65pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Classification Block}
\end{center}

\end{minipage}};
% Text Node
\draw (53,41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{65.88pt}\setlength\topsep{0pt}
\begin{center}
{\tiny (Pretrained) Embedding}
\end{center}

\end{minipage}};
% Text Node
\draw (251.9,145.9) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {${\textstyle \hat{f}(\boldsymbol{X} ,\ S)}$};
% Text Node
\draw (407.4,145.9) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {${\textstyle \hat{f}_{B}(\boldsymbol{X} ,\ S)}$};
% Text Node
\draw (282,41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{65.28pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Calibration Layer}
\end{center}

\end{minipage}};
% Text Node
\draw (250.5,157.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.62pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Unfair Scores}
\end{center}

\end{minipage}};
% Text Node
\draw (410.5,157.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{28.79pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Fair Scores}
\end{center}

\end{minipage}};

%Shape: Triangle [id:dp7949082877127149] 
\draw  [draw opacity=0][shading=_3ubsli8nm,_alay4xbbr] (178.44,167.8) -- (163,175.89) -- (163,159.71) -- cycle ;

\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 89; green, 89; blue, 89 }  ,fill opacity=1 ] (141.67,156.38) -- (162.9,156.38) -- (162.9,179.27) -- (141.67,179.27) -- cycle ;


% Text Node
\draw (145.8,161.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$S$};
% Text Node
\draw (85.82,115.42) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\boldsymbol{X}$};






\end{tikzpicture}

\vspace{-1cm}

